VSS: A Storage System for Video Analytics [Technical Report]

We present a new video storage system (VSS) designed to decouple high-level video operations from the low-level details required to store and efficiently retrieve video data. VSS is designed to be the storage subsystem of a video data management system (VDBMS) and is responsible for: (1) transparently and automatically arranging the data on disk in an efficient, granular format; (2) caching frequently-retrieved regions in the most useful formats; and (3) eliminating redundancies found in videos captured from multiple cameras with overlapping fields of view. Our results suggest that VSS can improve VDBMS read performance by up to 54%, reduce storage costs by up to 45%, and enable developers to focus on application logic rather than video storage and retrieval.

==> storage.tex <==

\section{Storage Manager}
\label{sec:storage-manager}



\begin{itemize}
\item Glob GOPs into large file + index like https://ieeexplore.ieee.org/document/5289196
\item \name section notes that the SM modifies the policies of overlapping videos to activate joint compression

\end{itemize}
